Coresets Meet EDCS: Algorithms for Matching and Vertex Cover on Massive Graphs

As massive graphs become more prevalent, there is a rapidly growing need for scalable algorithms that solve classical graph problems, such as maximum matching and minimum vertex cover, on large datasets. For massive inputs, several different computational models have been introduced, including the streaming model, the distributed communication model, and the massively parallel computation (MPC) model that is a common abstraction of MapReduce-style computation. In each model, algorithms are analyzed in terms of resources such as space used or rounds of communication needed, in addition to the more traditional approximation ratio. In this paper, we give a single unified approach that yields better approximation algorithms for matching and vertex cover in all these models. The highlights include: * The first one pass, significantly-better-than-2-approximation for matching in random arrival streams that uses subquadratic space, namely a $(1.5+\epsilon)$-approximation streaming algorithm that uses $O(n^{1.5})$ space for constant $\epsilon > 0$. * The first 2-round, better-than-2-approximation for matching in the MPC model that uses subquadratic space per machine, namely a $(1.5+\epsilon)$-approximation algorithm with $O(\sqrt{mn} + n)$ memory per machine for constant $\epsilon > 0$. By building on our unified approach, we further develop parallel algorithms in the MPC model that give a $(1 + \epsilon)$-approximation to matching and an $O(1)$-approximation to vertex cover in only $O(\log\log{n})$ MPC rounds and $O(n/poly\log{(n)})$ memory per machine. These results settle multiple open questions posed in the recent paper of Czumaj~et.al. [STOC 2018].

==> app-all.tex <==
\input{intro}

\input{prelim} 

\input{maximum-coreset}

\input{edcs}

\input{coresets}

\input{mpc-algorithms}

\clearpage
\appendix

\input{app-applications}

\input{app-prelim} 

==> coresets-short.tex <==


\section{Randomized Coresets for Matching and Vertex Cover}\label{short-sec:coresets-matching-vc}

In this short section, we introduce our randomized coresets for matching and vertex cover and sketch the proof of Result~\ref{short-res:coresets}. 
We show that one can compute an EDCS of the input graph $G$ by simply taking the union of the
EDCSes computed on each subgraph in the random $k$-partition. 
We then invoke Lemma \ref{short-lem:edcs} to obtain a large matching and a small vertex cover
of $G$ from this EDCS.

%These results are achieved by computing an EDCS of the input graph
%from an EDCS computed on each subgraph in the random $k$-partition and arguing that this EDCS can be used to recover a large matching and a small vertex cover of the input graph. % (by Lemmas~\ref{lem:edcs-matching} and~\ref{lem:edcs-vc}). 

% to argue that this EDCS allows for computing a large matching and a small vertex cover of the input graph. 

Let $G$ be any arbitrary graph and $\Gi{1},\ldots,\Gi{k}$ be a random $k$-partition of $G$. Our randomized coreset for both matching and vertex cover is simply any arbitrarily chosen EDCS of each $\Gi{i}$ with parameters 
$\beta = \polylog{(n)}$ and $\beta^- = \paren{1-\Theta((\eps/\log{n})^2)}\cdot \beta$. Since the maximum degree of any EDCS is at most $\beta$ by \propone of EDCS, size of this coreset
is only $O(n \cdot \beta) = \Ot(n)$. It thus only remains to prove the correctness of this coreset. % to finish the proof of Result~\ref{short-res:coresets}. 


Let $\Hi{i}$ be the EDCS computed on each graph $\Gi{i}$. The first part of the proof shows that $H:= \bigcup_{i=1}^{k} \Hi{i}$ 
is an EDCS for the original graph $G$ with parameters (roughly) equal to $(k \cdot \beta, k\cdot \beta^-)$ with high probability. This is intuitively true because by
Lemma~\ref{short-lem:edcs-edge-sampled}, the degree of every vertex $v$ across all subgraphs $\Hi{i}$ is essentially the same, so for any $i \in [k]$, we have 
$d_H(v) \approx k \cdot d_{\Hi{i}}(v)$.
As a result, for any edge $(u,v)$ in $\Hi{i}$ (for any $i \in [k]$),
\propone of EDCS $\Hi{i}$ ensures that
$\deg{H}{u} + \deg{H}{v} \approx k \cdot (\deg{\Hi{i}}{u} + \deg{\Hi{i}}{v}) \lesssim k \cdot \beta$,
so $(u,v)$ satisfies \propone of $H$ as well.
Similarly, every $(u,v) \in G \setminus H$ must be in $\Gi{i} \setminus \Hi{i}$ for some $i \in [k]$,
so by \proptwo of EDCS $\Hi{i}$ we have
$\deg{H}{u} + \deg{H}{v} \approx k \cdot (\deg{\Hi{i}}{u} + \deg{\Hi{i}}{v}) \gtrsim k \cdot \beta^-$.
So $(u,v)$ satisfies \proptwo of EDCS $H$ as well. 
See Lemma~\ref{lem:edcs-coreset} in the full version for the formal proof. 

%Let $\Hi{i}$ be the EDCS computed on each graph $\Gi{i}$. The first part of the proof shows that $H:= \bigcup_{i=1}^{k} \Hi{i}$ 
%is an EDCS for the original graph $G$ with parameters (roughly) equal to $(k \cdot \beta, k\cdot \beta^-)$ with high probability. This is intuitively true because by
%Lemma~\ref{short-lem:edcs-edge-sampled}, the degree of every vertex $v$ across all subgraphs $\Hi{i}$ is essentially the same and hence is within a factor $k$ of its degree in the final subgraph $H$. 
%As a result, for any edge $(u,v) \in \Hi{i}$ (for any $i \in [k]$), $\deg{H}{u} + \deg{H}{v} \geq k \cdot \beta$ by \propone of EDCS $\Hi{i}$ and hence this edge satisfies \propone of $H$ as well. 
%Similarly, one can also use the fact that every edge in $G$ appears in one of the subgraphs $\Gi{i}$ to argue that if $(u,v) \in \Gi{i} \setminus \Hi{i}$ (and hence is missing from $H$), 
%then $\deg{H}{u} + \deg{H}{v} \leq k \cdot \beta^-$, hence satisfying \proptwo of EDCS $H$ as well (see Lemma~\ref{lem:edcs-coreset} for the formal proof). 

We can now easily conclude the proof of Result~\ref{short-res:coresets}: 
since $H:= \bigcup_{i=1}^{k} \Hi{i}$ 
is an EDCS of the original graph $G$ with high probability, 
Lemma \ref{short-lem:edcs} guarantees that we can 
recover an (almost) $(3/2)$-approximate matching
and an (almost) $(2+\eps)$-approximate vertex cover for $G$ using only $H$.
see Theorems~\ref{thm:matching-edcs-coreset} and~\ref{thm:vc-edcs-coreset} in Section~\ref{sec:matching-vc-coreset} of the full version for formal proofs


%We can now conclude the proof easily. Since $H$ is an EDCS of the original graph with high probability, we can recover an (almost) $(3/2)$-approximate matching
%and an (almost) $(3+\eps)$-approximate vertex cover for $G$ using only $H$, i.e., the union of the coresets (by Lemmas~\ref{lem:edcs-matching} and~\ref{lem:edcs-vc}).
%This finalizes the proof sketch of Result~\ref{short-res:coresets} (see Theorems~\ref{thm:matching-edcs-coreset} and~\ref{thm:vc-edcs-coreset} in Appendix~\ref{sec:matching-vc-coreset} for formal proofs). 




==> edcs-short.tex <==
\negsp

\section{New Properties of Edge Degree Constrained Subgraphs} \label{short-sec:edcs}

We study further properties of EDCS in this section. Although EDCS was used prior to our work, \emph{all the properties proven in this section are entirely new to this paper} and look at the EDCS from a different vantage point. 
Previous work in~\cite{BernsteinS15,BernsteinS16} studied the EDCS from the perspective of how large of matching it contains and how it can be maintained efficiently in a dynamic graph. In this section, 
we prove several new structural properties of the EDCS itself. 
In particular, while it easy to see that in terms of edge-sets there
can be many different EDCSes of some fixed graph $G(V,E)$ 
(consider $G$ being a complete graph), we show that an EDCS is still ``semi-unique'' in that the degree distributions
of every EDCS (for the same $\beta$ and $\beta^-$) are almost the same.
In other words, the degree of any vertex $v$ is almost the same in every EDCS of $G$.
This is in sharp contrast with similar objects such as maximum matchings 
or $b$-matchings, which can vary a lot within the same graph. 

We now formally state the semi-uniqueness property
(Lemma \ref{short-lem:ddl}),
which is used it to show that the EDCS is
extremely robust under sampling and composition
(Lemmas \ref{short-lem:edcs-edge-sampled} and \ref{short-lem:edcs-vertex-sampled}). 

%In fact, our parallel algorithm 
%in Section~\ref{short-sec:mpc-algs} is \emph{entirely} based on these results and do not rely at all on the fact that an EDCS contains a large matching (i.e., do not depend on Lemma~\ref{short-lem:edcs} at all). 


 

%\subsection{Degree Distribution Lemma} \label{short-sec:edcs-ddl}

%Consider any two EDCS $A$ and $B$ of a graph $G(V,E)$. 

%It is easy to see that in general an EDCS of a graph $G(V,E)$ may not be unique (consider $G$ being a complete graph for example). 
%Remarkably, we show that despite this fact, the degree distribution of every EDCS of any arbitrary graph $G(V,E)$ is (almost) unique. In other words,
%the degree of any vertex $v \in V$ is almost the same across any two different EDCS of a graph $G$. This uniqueness of degree distribution is the crucial property that allows us 
%to combine arbitrarily chosen EDCS of sampled subgraphs to form an EDCS of the original graph. 

%\paragraph{Degree Distribution Lemma.} The following lemma proves the  semi-uniqueness of EDCS.

\begin{lemma}[{\bf Degree Distribution Lemma}]\label{short-lem:ddl}
	Fix a graph $G(V,E)$ and parameters $\beta,\beta^- = (1-\lambda) \cdot \beta$ (for $\lambda < 1/100$). For any two subgraphs $A$ and $B$ that are $\EDCS{G,\beta,\beta^-}$, and
	any vertex $v \in V$, $\card{\deg{A}{v} - \deg{B}{v}} = O(\log{n}) \cdot \lambda^{1/2} \cdot \beta.$
\end{lemma}

	%In the rest of this section, we fix the parameters $\beta,\beta^-$ and the two EDCS $A$ and $B$ in Lemma~\ref{lem:ddl}. 
\begin{proof}[Proof Sketch]	
	We start with a set $S_1$ of vertices that have 
	the most difference in degree between $A$ and $B$. For simplicity, assume vertex degrees are all larger by an additive factor of $\Delta$ in $A$ compared to $B$. 
	We look at all neighbors of $S_1$ in $A \setminus B$, denoted by $T_1$, and then all neighbors of $T_1$ in $B \setminus A$ plus the original set $S_1$ which we denote by $S_2$.  
	We then use the two properties of EDCS in Definition~\ref{short-def:edcs} to prove that the vertices in $S_2$ still have a larger degree in $A$ compared to $B$ by an additive
	factor which is only slightly smaller than $\Delta$, while the size of $S_2$ is a constant factor larger than $S_1$. The main observation behind this claim is that since vertices in $S$ have a ``large'' degree in $A$, their neighbors in $A \setminus B$ in $T_1$ should have a ``small'' degree to satisfy \propone of EDCS $A$. Similarly, since vertices in $S_1$ have a ``small'' degree in $B$, and since
	the edges in $A \setminus B$ are missing from the EDCS $B$, by \proptwo of EDCS $B$ the vertices in $T_1$ should have a ``large'' degree in $B$. Applying this idea one more time to 
	vertices in $T_1$ in order to obtain the set $S_2$, we can see that vertices in $S_2$ have a ``large'' degree in $A$ and a ``small'' degree in $B$, and that the decrease in the original gap $\Delta$ between the degree of vertices in $A$ vs $B$ is only $O(\beta - \beta^-) = O(\lambda \cdot \beta)$. 
	
	We use this argument repeatedly to construct the next set $S_3$ and so on.
	With each iteration the new set $S_i$
	is larger than the previous one $S_{i-1}$ by a constant \emph{multiplicative} factor, while the 
	$A$-vs.-$B$ degree gap only decreases by a small \emph{additive} factor from $S_{i-1}$ to $S_i$.
Now on one hand we can keep iterating this process as long as the $A$-vs.-$B$ degree gap remains $\geq \Delta$/2. On the other hand, a multiplicative increase in set size can only happen for $O(\log(n))$ steps before we run out of vertices. Thus, the gap must decrease from $\Delta$ to $\Delta/2$ after only $O(\log(n))$ steps of a small additive decrease, which gives us an upper bound on the original gap $\Delta$.
	
The formal proof is rather technical and is presented
in Section~\ref{sec:edcs-ddl} of the full version. 
\end{proof}	
%%	We now formalize this argument, starting with a technical lemma which allows us to 
%%obtain each set $S_i$ from the set $S_{i-1}$ in the above argument. 
%%	
%%\begin{lemma}\label{lem:ddl-increase}
%%	Fix an integer $D > 2\lambda^{1/2} \cdot \beta$ and suppose $S \subseteq V$ is such that for all $v \in S$, we have $\deg{A}{v} - \deg{B}{v} \geq D$. Then, there exists a set of 
%%	vertices $S' \supseteq S$ such that $\card{S'} \geq (1+2\lambda^{1/2}) \cdot \card{S}$ and for all $v \in S'$, $\deg{A}{v} - \deg{B}{v} \geq D - 2\lambda \cdot \beta$. 
%%\end{lemma}
%%\begin{proof}
%%	We define the following two sets $T$ and $T'$: 
%%	\begin{itemize}
%%		\item $T$ is the set of all neighbors of vertices in $S$ using \emph{only} the edges in $A \setminus B$. In other words, $T := \set{v \in V \mid \exists u \in S \wedge (u,v) \in A \setminus B}$.
%%		\item $T'$ is the set of all neighbors of vertices in $T$ using \emph{only} the edges in $B \setminus A$. In other words, $T' := \set{w \in V \mid \exists v \in T \wedge (v,w) \in B \setminus A}$. 
%%	\end{itemize}
%%
%%	We start by proving the following property on the degree of vertices in the sets $T$ and $T'$. %Roughly speaking, we expect the vertices in $T$ to have a higher degree in $B$ compared to $A$, and similarly vertices in $T'$
%%	\begin{claim}\label{clm:ddl-T}
%%		We have,
%%		\begin{itemize}
%%			\item for all $v \in T$,  $\deg{B}{v} - \deg{A}{v} \geq D - \lambda \cdot \beta$. 
%%			\item for all $w \in T'$, $\deg{A}{w} - \deg{B}{w} \geq D - 2\lambda \cdot \beta$. 
%%		\end{itemize}
%%	\end{claim}
%%	\begin{proof}
%%		For the first part, since $v \in T$, it means that there exists an edge $(u,v) \in A \setminus B$ such that $u \in S$. Since $(u,v)$ belongs to $A$, by $\propone$ of an EDCS we have 
%%		$\deg{A}{v} \leq \beta - \deg{A}{u} \leq \beta - \deg{B}{u} - D$. On the other hand, since $(u,v)$ does not belong to $B$, by $\proptwo$ of an EDCS we have
%%		$\deg{B}{v} \geq \beta - \lambda \cdot \beta - \deg{B}{u}$, completing the proof for vertices in $T$. 
%%		
%%		For the second part, since $w \in T'$, it means that there exists an edge $(v,w) \in B \setminus A$ such that $v \in T$. Since $(v,w)$ does not belong to $A$, by $\proptwo$ of an EDCS we have 
%%		$\deg{A}{w} \geq \beta - \lambda \cdot \beta - \deg{A}{v}$.  Moreover, since $(u,v)$ belongs to $B$, by $\propone$ of an EDCS, we have, $\deg{B}{w} \leq \beta  - \deg{B}{v}$. 
%%		This means that $\deg{A}{w} - \deg{B}{w} \geq \deg{B}{v} - \deg{A}{v} - \lambda \cdot \beta$ which is at least $D - 2\lambda \cdot \beta$ by the first part. 
%%	\end{proof}
%%	
%%	Notice that since $D > 2\lambda \cdot \beta$, by Claim~\ref{clm:ddl-T}, for any vertex $v \in T$, we have $\deg{B}{v} > \deg{A}{v}$ and hence $S \cap T = \emptyset$ (similarly, $T \cap T' = \emptyset$, but $S$ and $T'$ may intersect). 
%%	We define the set $S'$ in the lemma statement to be $S' := S \cup T'$. The bound on the degree of vertices in $S'$ follows immediately from Claim~\ref{clm:ddl-T} (recall that vertices in $S$ already satisfy the degree requirement for the set $S'$). 
%%	In the following, we show that $\card{T' \setminus S} \geq 2\lambda^{1/2} \cdot \card{S}$, which finalizes the proof. 
%%	
%%	Recall that  $E_{A \setminus B}(S)$ and $E_{A \setminus B}(S,T)$ denote the set of edges in subgraph $A \setminus B$ incident on vertices $S$, and between vertices $S$ and $T$, respectively. 
%%	We have, 
%%	\begin{align*}
%%		\card{E_{B \setminus A}(T,T' \setminus S)} &= \card{E_{B \setminus A}(T)} - \card{E_{B \setminus A}(T,S)} \tag{as all the edges in $B \setminus A$ that are incident on $T$ are going to $T'$}\\
%%		&\geq \card{E_{A \setminus B}(T)} - \card{E_{B \setminus A}(T,S)}  \tag{as by Claim~\ref{clm:ddl-T}, the degree of vertices in $T$ is larger in $B \setminus A$ compared to $A \setminus B$} \\
%%		&\geq \card{E_{A \setminus B}(S)} - \card{E_{B \setminus A}(S)} \tag{as all edges in $A \setminus B$ incident on $S$ are also incident on $T$}  \\
%%		&\geq \card{S} \cdot D \tag{by the assumption on the degree of vertices in $S$ in subgraphs $A$ and $B$}
%%	\end{align*}
%%	
%%	Finally, since $B$ is an EDCS, the maximum degree of any vertex in $T' \setminus S$ is at most $\beta$ and hence there should be at least $\card{S} \cdot \frac{D}{\beta} \geq 2\lambda^{1/2} \cdot \card{S}$ vertices in $T' \setminus S$  
%%	(as $D > 2\lambda^{1/2}\cdot \beta$). 
%%\end{proof}
%%
%%%We are now ready to prove Lemma~\ref{lem:ddl}. 
%%
%%\begin{proof}[Proof of Lemma~\ref{lem:ddl}]
%%	Suppose towards a contradiction that there exists a vertex $v \in V$ s.t. $D := \deg{A}{v} - \deg{B}{v} \geq 3\ln{(n)} \cdot \lambda^{1/2}\cdot \beta$ (the other case is symmetric). Let $D_0 = D$ and $S_0 = \set{v}$ and 
%%	for $i = 1$ to $t:=\lambda^{-1/2} \cdot \paren{{\ln{(n)}+1}}$: define the set $S_i$ and integer $D_i$ by applying Lemma~\ref{lem:ddl-increase} to $S_{i-1}$ and $D_{i-1}$ (i.e., $S_i = S'$ and $D_i = D_{i-1} - 2\lambda \cdot \beta$). 
%%	By the lower bound on the value of $D$, for any 
%%	$i \in [t]$, we have that $D_i \geq D - i \cdot 2\lambda \cdot \beta > 2\lambda^{1/2} \cdot \beta$, and hence we can indeed apply Lemma~\ref{lem:ddl-increase}. As a result, we have, 
%%	\begin{align*}
%%		\card{S_{t}} \geq \paren{1+2\lambda^{1/2}} \cdot \card{S_{t-1}} \geq \paren{1+2\lambda^{1/2}}^{t} \cdot \card{S_0} \geq \exp{\paren{\lambda^{1/2} \cdot t}} > \exp\paren{\ln{(n)}} = n.
%%	\end{align*}
%%	which is a contradiction as there are only $n$ vertices in the graph $G$. Consequently, we obtain that for any vertex $v$, $\card{\deg{A}{v} - \deg{B}{v}} = O(\log{n}) \cdot \lambda^{1/2} \cdot \beta$, finalizing the proof.  
%%	%, whereby for all $v \in S_i$, $\deg{A}{v} - \deg{B}{v} \geq D_i$ with $D_i := D_{i-1} - 2\lambda \cdot \beta$. 
%%\end{proof}

\paragraph{EDCS in Sampled Subgraphs.}% \label{sec:edcs-sampled}
We use the Degree Distribution Lemma to prove two lemmas regarding EDCS in sampled subgraphs. The first concerns edge sampled subgraphs. We show that the degree distributions of any two EDCS for 
two different edge sampled subgraphs of $G$ is almost the same no matter how the two EDCS are selected or even if the choice of the two subgraphs are \emph{not} independent. This Lemma is used in our Result \ref{short-res:coresets} on randomized coresets (see Section \ref{short-sec:coresets-matching-vc}).

\begin{lemma}[EDCS in Edge Sampled Subgraphs] \label{short-lem:edcs-edge-sampled}
	Fix any graph $G(V,E)$ and $p \in (0,1)$. Let $G_1$ and $G_2$ be two \emph{edge sampled subgraphs} of $G$ with probability $p$ (chosen \emph{not} necessarily independently). Let $H_1$ and $H_2$ be 
	arbitrary EDCSs of $G_1$ and $G_2$ with parameters $\paren{\beta, (1-\lambda) \cdot \beta}$. Suppose $\beta \geq 750 \cdot \lambda^{-2} \cdot \ln{(n)}$, then, with probability $1-4/n^9$, simultaneously for all $v \in V$: 
	\begin{align*}
		\card{\deg{H_1}{v} - \deg{H_2}{v}} \leq O(\log{n}) \cdot \lambda^{1/2} \cdot \beta. 
	\end{align*}
\end{lemma}

We also prove a qualitatively similar lemma for \emph{vertex sampled} subgraphs. This is needed in Result \ref{short-res:mpc} for parallel algorithms (see Section \ref{short-sec:mpc-algs}).
The main difference from edge sampling is that there will be a huge gap between the degree of a vertex between the two EDCS if it is sampled in one subgraph but not the other. However, we show that the degree of vertices that are sampled in \emph{both} subgraphs are still almost the same. % across the two different (and arbitrarily chosen) EDCS for the subgraphs.  

\begin{lemma}[EDCS in Vertex Sampled Subgraphs]\label{short-lem:edcs-vertex-sampled}
	Fix any graph $G(V,E)$ and $p \in (0,1)$. Let $G_1$ and $G_2$ be two \emph{vertex sampled subgraphs} of $G$ with probability $p$ (chosen \emph{not} necessarily independently). Let $H_1$ and $H_2$ be 
	arbitrary EDCSs of $G_1$ and $G_2$ with parameters $\paren{\beta, (1-\lambda)\beta}$. If $\beta \geq 750 \cdot \lambda^{-2} \cdot \ln{(n)}$, then, with probability $1-4/n^9$, simultaneously for all $v \in G_1 \cap G_2$: 
	\begin{align*}
		\card{\deg{H_1}{v} - \deg{H_2}{v}} \leq O(\log{n}) \cdot \lambda^{1/2} \cdot \beta. 
	\end{align*}
\end{lemma}

The proofs of both these lemmas proceed along the following lines. We start with any EDCS $H$ of the original graph $G$ with parameters (almost) $\paren{\beta/p,\beta^-/p}$.  We then consider the set of edges from $H$ in each of the sampled
subgraphs $G_1$ and $G_2$, i.e., the two subgraphs $H'_1 := G_1 \cap H$ and $H'_2 := G_2 \cap H$. We use the randomness in the process of sampling subgraphs $G_1$ and $G_2$ to prove that, with high probability, $H'_1$ and $H'_2$ are both an
EDCS of $G_1$ and $G_2$, respectively, with parameters $\paren{\beta,\beta^-}$.
Moreover, since they are sampled from the same underlying EDCS $H$, $H'_1$ and $H'_2$ end
up having similar degree distributions (denoted by $H'_1 \sim H'_2$).
Finally, we use our degree distribution lemma (Lemma~\ref{short-lem:ddl}) to argue that for any arbitrary EDCS $H_1$ of $G_1$ and $H_2$ of $G_2$,
degree distribution of $H_1$ (resp. $H_2$) is close to $H'_1$ (resp. $H'_2$), namely $H_1 \sim H'_1$ and $H_2 \sim H'_2$.
We thus have $H_1 \sim H'_1 \sim H'_2 \sim H_2$, completing the proof. 
The formal proofs of these two lemmas are deferred to Section~\ref{sec:edcs} of the full version. 

%%There are some technical differences in implementing the above intuition between the edge sampled and vertex sampled subgraphs and hence we provide a separate proof for each case.  
%%
%%
%%\subsubsection{EDCS in Edge Sampled Subgraphs: Proof of Lemma~\ref{lem:edcs-edge-sampled}}
%%\begin{proof}[Proof of Lemma~\ref{lem:edcs-edge-sampled}]
%%	We first prove that edge sampling an EDCS results in another EDCS for the sampled subgraph. 
%%	 
%%	\begin{claim}\label{clm:edcs-edge-sampled}
%%		Let $H$ be an $\EDCS{G,\beta_H,\beta^-_H}$ for parameters $\beta_H := (1-\frac{\lambda}{2}) \cdot \frac{\beta}{p}$ and $\beta^-_H := \beta_H-1$. 
%%		Suppose $G_p := G^E_p(V,E_p)$ is an edge sampled subgraph of $G$ and $H_p := H \cap G_p$; then, with probability $1-2/n^9$: 
%%		\begin{enumerate}
%%			\item For any vertex $v \in V$, $\card{\deg{H_p}{v} - p \cdot \deg{H}{v}} \leq \frac{\lambda}{5} \cdot \beta$.
%%			\item $H_p$ is an EDCS of $G_p$ with parameters $\paren{\beta,(1-\lambda) \cdot \beta}$.  
%%		\end{enumerate}
%%	\end{claim}
%%	\begin{proof}
%%	For any vertex $v \in V$, $\Ex{\bracket{\deg{H_p}{v}}} = p \cdot \deg{H}{v}$ and 
%%	$\deg{H}{v} \leq \beta_H$ by $\propone$ of EDCS $H$. Moreover, since each neighbor of $v$ in $H$ is sampled in $H_p$ independently, by Chernoff bound (Proposition~\ref{prop:chernoff}), we have, 
%%	\begin{align*}
%%		\Pr\paren{\card{\deg{H_p}{v} - p \cdot \deg{H}{v}} \geq \frac{\lambda}{5} \cdot \beta} \leq 2\cdot \exp\paren{-\frac{\lambda^2  \cdot \beta}{75}}  \leq 2\cdot \exp\paren{-10\ln{n}} = \frac{2}{n^{10}},
%%	\end{align*}
%%	where the second inequality is by the lower bound on $\beta$ in Lemma~\ref{lem:edcs-vertex-sampled} statement. 
%%	In the following, we condition on the event that: 
%%	\begin{align}
%%		\forall v \in V~~ \card{\deg{H_p}{v} - p \cdot \deg{H}{v}} \leq \frac{\lambda}{5} \cdot \beta. \label{eq:edge-degree-event}
%%	\end{align}
%%	This event happens with probability at least $1-2/n^9$ by above equation and a union bound on $\card{V} = n$ vertices. This finalizes the proof of the first part of the claim. 
%%	We are now ready to prove that $H_p$ is indeed an $\EDCS{G_p,\beta,(1-\lambda)\cdot \beta}$ conditioned on this event. 
%%	
%%	Consider any edge $(u,v) \in H_p$. Since $H_p \subseteq H$, $(u,v) \in H$ as well. Hence, we have, 
%%	\begin{align*}
%%		\deg{H_p}{u} + \deg{H_p}{v} \Leq{Eq~(\ref{eq:edge-degree-event})} p \cdot \Paren{\deg{H}{u} + \deg{H}{v}} + \frac{2\lambda}{5} \cdot \beta \leq p \cdot \beta_H +  \frac{2\lambda}{5} \cdot \beta  
%%		= (1-\frac{\lambda}{2}) \cdot \beta + \frac{2\lambda}{5} \cdot \beta < \beta,
%%	\end{align*}
%%	where the second inequality is by \propone of EDCS $H$ and the equality is by the choice of $\beta_H$. As a result, $H_p$ satisfies \propone of EDCS for parameter $\beta$.
%%	
%%	Now consider an edge $(u,v) \in G_p \setminus H_p$. Since $H_p = G_p \cap H$,  $(u,v) \notin H$ as well. Hence,  
%%	\begin{align*}
%%		\deg{H_p}{u} + \deg{H_p}{v} &\Geq{Eq~(\ref{eq:edge-degree-event})} p \cdot \Paren{\deg{H}{u} + \deg{H}{v}} - \frac{2\lambda}{5} \cdot  \beta \geq p \cdot \beta^-_H - \frac{2\lambda}{5} \cdot  \beta \\
%%		&= (1-\frac{\lambda}{2}) \cdot \beta - p - \frac{2\lambda}{5} \cdot \beta 
%%		> (1-\lambda) \cdot \beta,
%%	\end{align*}
%%	where the second inequality is by \proptwo of EDCS $H$ and the equality is by the choice of $\beta^-_H$. 
%%	As such, $H_p$ satisfies \proptwo of EDCS for parameter $(1-\lambda) \cdot \beta$ and hence $H_p$ is indeed an $\EDCS{G_p,\beta,(1-\lambda) \cdot \beta}$. 
%%	\end{proof}
%%	
%%	We continue with the proof of Lemma~\ref{lem:edcs-edge-sampled}. 
%%	%We can now use Claim~\ref{clm:edcs-vertex-sampled} together with Lemma~\ref{lem:ddl} to finalize the proof. 
%%	Let $H$ be an $\EDCS{G,\beta_H,\beta^-_H}$ for the parameters $\beta_H,\beta_H^-$ in Claim~\ref{clm:edcs-edge-sampled}. The existence of $H$ follows from Lemma~\ref{lem:edcs-exists} as $\beta_H^- < \beta_H$. 
%%	Define $\hH_{1} := H \cap G_1$ and $\hH_{2} := H \cap G_2$. By Claim~\ref{clm:edcs-edge-sampled}, $\hH_{1}$ (resp. $\hH_{2}$) is an EDCS of $G_1$ (resp. $G_2$) with parameters $\paren{\beta,(1-\lambda)\beta}$ with
%%	probability $1-4/n^9$. In the following, we condition on this event. 
%%	 
%%	By Lemma~\ref{lem:ddl} (Degree Distribution Lemma), since both $H_{1}$ (resp. $H_2$) and $\hH_1$ (resp. $\hH_2$) are EDCS for $G_1$ (resp. $G_2$), the degree of vertices in both of them should be ``close'' to each other. Moreover, since
%%	by Claim~\ref{clm:edcs-vertex-sampled} the degree of each vertex in $\hH_1$ and $\hH_2$ is close to $p$ times its degree in $H$, we can argue that the vertex degrees in $H_1$ and $H_2$ are close. Formally, 
%%	for any $v \in V$, we have, 
%%	\begin{align*}
%%		\card{\deg{H_1}{v} - \deg{H_2}{v}} &\leq \card{\deg{H_1}{v} - \deg{\hH_1}{v}} + \card{\deg{\hH_1}{v} - \deg{\hH_2}{v}} + \card{\deg{\hH_2}{v} - \deg{H_2}{v}}  \\
%%		&\!\!\!\!\!\!\!\!\!\Leq{Lemma~\ref{lem:ddl}} O(\log{n}) \cdot \lambda^{1/2} \cdot \beta + \card{\deg{\hH_1}{v} - p \cdot \deg{H}{v}} + \card{\deg{\hH_2}{v} - p \cdot \deg{H}{v}} \\
%%		&\!\!\!\!\!\!\!\!\Leq{Claim~\ref{clm:edcs-edge-sampled}} O(\log{n}) \cdot \lambda^{1/2} \cdot \beta + O(1) \cdot \lambda \cdot \beta,
%%	\end{align*}
%%	finalizing the proof. 
%%\end{proof}
%%
%%\subsubsection{EDCS in Vertex Sampled Subgraphs: Proof of Lemma~\ref{lem:edcs-vertex-sampled}}
%%\begin{proof}[Proof of Lemma~\ref{lem:edcs-vertex-sampled}]
%%
%%
%%	We first prove that vertex sampling an EDCS results in another EDCS for the sampled subgraph. 
%%	 
%%	\begin{claim}\label{clm:edcs-vertex-sampled}
%%		Let $H$ be an $\EDCS{G,\beta_H,\beta^-_H}$ for parameters $\beta_H := (1-\frac{\lambda}{2}) \cdot \frac{\beta}{p}$ and $\beta^-_H := \beta_H - 1$. 
%%		Suppose $G_p := G^V_p(V_p,E_p)$ is a vertex sampled subgraph of $G$ and $H_p := H \cap G_p$; then, with probability $1-2/n^9$: 
%%		\begin{enumerate}
%%			\item For any vertex $v \in V_p$, $\card{\deg{H_p}{v} - p \cdot \deg{H}{v}} \leq \frac{\lambda}{5} \cdot \beta$.
%%			\item $H_p$ is an EDCS of $G_p$ with parameters $\paren{\beta,(1-\lambda) \cdot \beta}$.  
%%		\end{enumerate}
%%	\end{claim}
%%	\begin{proof}
%%	For any vertex $v \in V_p$, $\Ex{\bracket{\deg{H_p}{v}}} = p \cdot \deg{H}{v}$ by the independent sampling of vertices and 
%%	$\deg{H}{v} \leq \beta_H$ by \propone of EDCS $H$. Moreover, since each neighbor of $v$ in $H$ is sampled in $H_p$ independently, by Chernoff bound (Proposition~\ref{prop:chernoff}), we have, 
%%	\begin{align*}
%%		\Pr\paren{\card{\deg{H_p}{v} - p \cdot \deg{H}{v}} \geq \frac{\lambda}{5} \cdot \beta} \leq 2\cdot \exp\paren{-\frac{\lambda^2  \cdot \beta}{75}}  \leq 2\cdot \exp\paren{-10\ln{n}} = \frac{2}{n^{10}},
%%	\end{align*}
%%	where the second inequality is by the lower bound on $\beta$ in Lemma~\ref{lem:edcs-vertex-sampled} statement. 
%%	In the following, we condition on the event that: 
%%	\begin{align}
%%		\forall v \in V_p~~ \card{\deg{H_p}{v} - p \cdot \deg{H}{v}} \leq \frac{\lambda}{5} \cdot \beta. \label{eq:vertex-degree-event}
%%	\end{align}
%%	which happens with probability at least $1-2/n^9$ by above equation and a union bound on $\card{V_p} \leq n$ vertices. This finalizes the proof of the first part of the claim. 
%%	We are now ready to prove that $H_p$ is indeed an $\EDCS{G_p,\beta,(1-\lambda)\cdot \beta}$ conditioned on this event. 
%%	
%%	Consider any edge $(u,v) \in H_p$. Since $H_p \subseteq H$, $(u,v) \in H$ as well. Hence, we have, 
%%	\begin{align*}
%%		\deg{H_p}{u} + \deg{H_p}{v} \Leq{Eq~(\ref{eq:vertex-degree-event})} p \cdot \Paren{\deg{H}{u} + \deg{H}{v}} + \frac{2\lambda}{5} \cdot \beta \leq p \cdot \beta_H +  \frac{2\lambda}{5} \cdot \beta  
%%		= (1-\frac{\lambda}{2}) \cdot \beta + \frac{2\lambda}{5} \cdot \beta < \beta,
%%	\end{align*}
%%	where the second inequality is by \propone of EDCS $H$ and the equality is by the choice of $\beta_H$. As a result, $H_p$ satisfies \propone of EDCS for parameter $\beta$.
%%	
%%	Now consider an edge $(u,v) \in G_p \setminus H_p$. Since $H_p = G_p \cap H$,  $(u,v) \notin H$ as well. Hence,  
%%	\begin{align*}
%%		\deg{H_p}{u} + \deg{H_p}{v} &\Geq{Eq~(\ref{eq:vertex-degree-event})} p \cdot \Paren{\deg{H}{u} + \deg{H}{v}} - \frac{2\lambda}{5} \cdot  \beta \geq p \cdot \beta^-_H - \frac{2\lambda}{5} \cdot  \beta \\
%%		&= (1-\frac{\lambda}{2}) \cdot \beta - p - \frac{2\lambda}{5} \cdot \beta 
%%		> (1-\lambda) \cdot \beta,
%%	\end{align*}
%%	where the second inequality is by \proptwo of EDCS $H$ and the equality is by the choice of $\beta^-_H$. 
%%	As such, $H_p$ satisfies \proptwo of EDCS for parameter $(1-\lambda) \cdot \beta$ and hence $H_p$ is indeed an $\EDCS{G_p,\beta,(1-\lambda) \cdot \beta}$. 
%%	\end{proof}
%%	
%%	We continue with the proof of Lemma~\ref{lem:edcs-vertex-sampled}. 
%%	%We can now use Claim~\ref{clm:edcs-vertex-sampled} together with Lemma~\ref{lem:ddl} to finalize the proof. 
%%	Let $H$ be an $\EDCS{G,\beta_H,\beta^-_H}$ for the parameters $\beta_H,\beta_H^-$ in Claim~\ref{clm:edcs-vertex-sampled}. The existence of $H$ follows from Lemma~\ref{lem:edcs-exists} as $\beta^-_H < \beta_H$. 
%%	Define $\hH_{1} := H \cap G_1$ and $\hH_{2} := H \cap G_2$. By Claim~\ref{clm:edcs-vertex-sampled}, $\hH_{1}$ (resp. $\hH_{2}$) is an EDCS of $G_1$ (resp. $G_2$) with parameters $\paren{\beta,(1-\lambda)\beta}$ with
%%	probability $1-4/n^9$. In the following, we condition on this event. 
%%	 
%%	By Lemma~\ref{lem:ddl} (Degree Distribution Lemma), since both $H_{1}$ (resp. $H_2$) and $\hH_1$ (resp. $\hH_2$) are EDCS for $G_1$ (resp. $G_2$), the degree of vertices in both of them should be ``close'' to each other. Moreover, since
%%	by Claim~\ref{clm:edcs-vertex-sampled} the degree of each vertex in $\hH_1$ and $\hH_2$ is close to $p$ times its degree in $H$, we can argue that the degree of shared vertices in $H_1$ and $H_2$ are close. Formally, 
%%	let $v$ be a vertex in both $G_1$ and $G_2$; we have, 
%%	\begin{align*}
%%		\card{\deg{H_1}{v} - \deg{H_2}{v}} &\leq \card{\deg{H_1}{v} - \deg{\hH_1}{v}} + \card{\deg{\hH_1}{v} - \deg{\hH_2}{v}} + \card{\deg{\hH_2}{v} - \deg{H_2}{v}}  \\
%%		&\!\!\!\!\!\!\!\!\!\Leq{Lemma~\ref{lem:ddl}} O(\log{n}) \cdot \lambda^{1/2} \cdot \beta + \card{\deg{\hH_1}{v} - p \cdot \deg{H}{v}} + \card{\deg{\hH_2}{v} - p \cdot \deg{H}{v}} \\
%%		&\!\!\!\!\!\!\!\!\Leq{Claim~\ref{clm:edcs-vertex-sampled}} O(\log{n}) \cdot \lambda^{1/2} \cdot \beta + O(1) \cdot \lambda \cdot \beta,
%%	\end{align*}
%%	finalizing the proof. 
%%\end{proof}



==> intro-short.tex <==
\section{Introduction}\label{short-sec:intro}

As massive graphs become more prevalent, there is a rapidly growing
need for scalable algorithms that  solve classical
graph problems on large datasets.
 When dealing with massive data,
the entire input graph is orders of magnitude larger than the amount of storage
on one processor and hence any algorithm needs to explicitly address
this issue.
For massive inputs, several different computational models
have been introduced, each focusing on certain additional resources needed
to solve large-scale problems.
Some examples include the streaming model,
the distributed communication model, and the
{massively parallel computation (MPC)} model that is a common
abstraction of MapReduce-style computation (see Section~\ref{short-sec:prelim}
for a definition of MPC). The target resources in these models are the number
of rounds of communication and the local storage
on each machine.



Given the variety of relevant models, there has been a lot of
attention on designing general algorithmic techniques that can
be applicable across a wide range of settings.  We focus on this task
for two prominent graph optimization problems: maximum matching
and minimum vertex cover.  Our main result (Section
\ref{short-sec:result1}) presents a \textbf{\emph{single unified algorithm}}
that immediately implies significantly improved results (in some or all of the parameters involved) for both
problems in all three models discussed above. For example, in
{random arrival order} streams, our algorithm computes a $(1.5+\eps)$-approximate matching in a single pass with
$\Ot(n^{1.5})$ space; this significantly improves upon the approximation ratio of previous
single-pass algorithms using subquadratic space, and is the first result
to present strong evidence of a separation between random and
adversarial order for matching. Another example is in the MPC model:
Given $\Ot(n^{1.5})$ space per machine, our algorithm computes a $(1.5+\eps)$-approximate matching in only 2 MPC rounds; this
significantly improves upon all previous results with a small constant
number of rounds.

Our algorithm is built on the framework of randomized composable
  coreset, which was recently suggested by Assadi and
Khanna~\cite{AssadiK17} as a means to unify different models for
processing massive graphs (see Section \ref{short-sec:coreset}).  A
common drawback of unified approaches is that although they have the
advantage of versatility, the results they yield are often not as
strong as those that are tailored to one particular model. It is
therefore perhaps surprising that we can design essentially a single
algorithm that improves upon the state-of-the-art algorithms in all
three models discussed above simultaneously. Our approach for the
matching problem notably goes significantly beyond a
$2$-approximation, which is a notorious barrier for matching in all
the models discussed above.


We also build on our techniques to achieve a second result (Section
\ref{short-sec:result2}) particular to the MPC model. We show that
when each machine has only $O(n)$ space (or even $O(n/\polylog(n)))$,
$O(\log\log{n})$ rounds suffice to compute a $(1+\eps)$-approximate
matching or a $O(1)$-approximate vertex cover. This improves
significantly upon the recent breakthrough of Czumaj et
al. \cite{CzumajLMMOS17}, which does not extend to vertex cover, and
requires $O(\log\log^2(n))$ rounds. Our results in this part settle
multiple open questions posed by Czumaj~\etal~\cite{CzumajLMMOS17}.


\subsection{Randomized Composable Coresets}
\label{short-sec:coreset} 



Two examples of general techniques widely used for processing massive data sets are 
linear sketches (see e.g. ~\cite{AhnGM12Linear,AGM12,KapralovLMMS14,AssadiKLY16,ChitnisCEHMMV16,BulteauFKP16,KW14,BhattacharyaHNT15,McGregorTVV15}) and composable coresets
(see e.g.~\cite{BadanidiyuruMKK14,BalcanEL13,BateniBLM14,IndykMMM14,MirzasoleimanKSK13,MirrokniZ15,AssadiK17}).
Both proceed by arbitrarily partitioning the data into smaller pieces,
computing a small-size summary of each piece, and then showing that these summaries can be combined
into a small-size summary of the original data set. This approach has a wide range of applications,
but strong impossibility results are known for both techniques for the two problems of {maximum matching} and {minimum vertex cover} that we study in this paper~\cite{AssadiKLY16}.

Recently, Assadi and Khanna~\cite{AssadiK17} turned to the notion of randomized composable coresets---originally introduced in the context of submodular maximization by Mirrokni and Zadimoghadam~\cite{MirrokniZ15} (see also~\cite{BarbosaENW15})---to bypass these strong impossibility results. 
The idea is to partition the graph into \emph{random} pieces rather than arbitrary ones. 
The authors in \cite{AssadiK17}
designed randomized composable coresets for matching and vertex cover, but although
this led to unified algorithms for many models of computation, the resulting bounds were
still for the most part weaker than the state-of-the-art algorithms tailored to each particular model. 

We now define randomized composable coresets in more detail; for brevity, we refer to them as randomized coresets.
Given a graph $G(V,E)$, with $m=|E|$ and $n=|V|$,  consider a random partition of $E$ into $k$ edge sets
$\set{\Ei{1},\ldots,\Ei{k}}$; each edge in $E$ is sent to exactly one of the $\Ei{i}$,
picked uniformly at random, thereby partitioning graph $G$ into $k$ subgraphs 
$\Gi{i}(V, \Ei{i})$. 


\begin{definition}[Randomized Composable Coreset~\cite{MirrokniZ15,AssadiK17}]
\label{short-def:randomized-coreset}
Consider an algorithm $\core$ that takes as input an arbitrary graph and returns a 
\textbf{subgraph} $\core(G) \subseteq G$. $\core$ is said to output an $\alpha$-approximate randomized coreset for maximum matching if given any graph $G(V,E)$ and a random $k$-partition of $G$ into $\Gi{i}(V,\Ei{i})$, the size of the maximum matching
in $\core(\Gi{1}) \cup \ldots \cup \core(\Gi{k})$ is an $\alpha$-approximation to the size of the maximum matching in $G$ with high probability.
We refer to the \textbf{number of edges} in the returned subgraph by $\core$ as the \textbf{size} of the coreset. 
Randomized coresets are defined analogously for minimum vertex cover and other graph problems. 
\end{definition}

It is proven in~\cite{AssadiK17} that any $O(1)$-approximate randomized coreset for matching or vertex cover has size $\Omega(n)$. Thus, similarly to~\cite{AssadiK17}, we focus
on designing randomized coresets of size $\Ot(n)$, which is optimal within logarithmic factors. 
Any $\alpha$-approximate randomized
coreset of size $\Ot(n)$ for matching or vertex cover immediately yields the following algorithms for these problems on a graph $G(V,E)$ with $n$ vertices and $m$ edges: (see Proposition~\ref{prop:coreset-application} for more details and proofs.)  

\begin{itemize}
	\item \textbf{Streaming:} An $\alpha$-approximation single-pass streaming algorithm on {random arrival} streams using $\Ot(\sqrt{mn} + n) = \Ot(n^{1.5}$) space. 
	\item \textbf{MPC:} An $\alpha$-approximation MPC algorithm in two rounds with $O(\sqrt{m/n})$ machines, each with $\Ot(\sqrt{mn} + n) = \Ot(n^{1.5}$) memory. 
	\item \textbf{Distributed:} An $\alpha$-approximation simultaneous communication protocol on {randomly partitioned} inputs using $\Ot(n)$ communication per machine/player. 
\end{itemize}

%\noindent See Proposition~\ref{prop:coreset-application} for more details and proofs.
%%
%%
%%\begin{proposition}\label{short-prop:coreset-application}
%%Suppose $\core$ outputs an $\alpha$-approximate randomized coreset of size $\ot(n)$ for problem $P$ (e.g. matching).
%%Let $G(V,E)$ be a graph with $m = \card{E}$ edges. This yields:
%%	\begin{enumerate}
%%		\item A parallel algorithm in the MPC model that with high probability outputs an $\alpha$-approximation to $P$ in two rounds with $O(\sqrt{m/n})$ machines, each with $O(\sqrt{mn} + n) = O(n^{1.5}$) memory. 
%%		\item A streaming algorithm that on \emph{random arrival} streams outputs an $\alpha$-approximation to $P(G)$ with high probability using $O(\sqrt{mn}) = O(n^{1.5}$) space. 
%%		\item A simultaneous communication protocol that on \emph{randomly partitioned} inputs computes an $\alpha$-approximation to $P(G)$ with high probability using $\ot(n)$ communication per machine/player. 
%%	\end{enumerate}
%%\end{proposition}


\subsection{First Result: Improved Algorithms via a New Randomized Coreset}
\label{short-sec:result1}

%We start by studying the previous randomized coreset of~\cite{AssadiK17} for matching, which was simply to pick a maximum matching of each
%machine's subgraph as its coreset. This is arguably the most natural approach to the problem and results in truly sparse subgraphs
%(maximum degree one). As a warm-up to our main results, we present a simpler and improved analysis (compared to that in~\cite{AssadiK17}), which shows that this coreset
%achieves a $3$-approximation (vs. $9$-approximation proven in~\cite{AssadiK17}). We also show that there exist graphs on which the approximation ratio of this coreset
%is at least $2$. This suggests that to achieve a better than $2$ approximation, fundamentally different ideas are needed
%which brings us to our first main result. 
%\smallskip

As our first result, we develop a new randomized composable coreset for matching and vertex cover. 

\begin{result}\label{short-res:coresets}
	There exist randomized composable coresets of size $\Ot(n)$ that for any constant $\eps > 0$, give a $(3/2+\eps)$-approximation for maximum matching and a $(2+\eps)$-approximation for minimum vertex cover with high probability. 
\end{result}

\noindent Our results improve upon the randomized coresets
of~\cite{AssadiK17} that obtained $O(1)$ and $O(\log{n})$
approximation to matching and vertex cover, respectively.  
Our approach is entirely different, and in particular we go
beyond the ubiquitous 2-approximation barrier for matching (in Section~\ref{sec:maxmatching-lower} 
of the full version, we show that the previous approach 
of ~\cite{AssadiK17} provably cannot go below $2$.). Result~\ref{short-res:coresets}
  yields a unified framework that improves upon the state-of-the art algorithms for matching and vertex cover across several
  computational models, for some or all the parameters involved.
%Let us exhibit the most interesting results.

\paragraph{\underline{First implication: streaming.}} 

We consider single-pass streaming algorithms. Computing a $2$-approximation for matching (and vertex cover) in $O(n)$ space is
trivial: simply maintain a maximal matching. Going beyond this barrier has 
remained one of the central open questions in the graph streaming literature since the introduction of the field~\cite{FKMSZ05}.
No $o(n^2)$-space algorithm is known for this task on {adversarially ordered} streams and the 
lower bound result by Kapralov~\cite{Kapralov13} (see also~\cite{GoelKK12}) proves that an $\paren{\frac{e}{e-1}}$-approximation requires $n^{1+\Omega(1/\log\log{n})}$ space.
To make progress on this fascinating open question, Konrad~\etal~\cite{KonradMM12} suggested the study of matching in \emph{random arrival} streams. They presented 
an algorithm with approximation ratio strictly better than $2$, namely $2-\delta$ for $\delta \approx 0.002$, in $O(n)$ space over random streams. 
A direct application of our Result~\ref{short-res:coresets} improves the approximation ratio of this algorithm significantly albeit at a cost of a larger space requirement. 
\begin{corollary}\label{short-cor:coreset-stream}
	There exists a single-pass streaming algorithm on random arrival streams that uses $\Ot(n^{1.5})$ space and with high probability (over the randomness of the stream) achieves a $(3/2+\eps)$-approximation
	to the maximum matching problem for constant $\eps > 0$. 
\end{corollary}

Our results provide the first strong evidence of a separation between random-order and
adversarial-order streams for matching, as it is the first algorithm that beats 
the ratio of $\paren{\frac{e}{e-1}}$, which is known to be ``hard'' on adversarial streams ~\cite{Kapralov13}.
Although the lower bound of ~\cite{Kapralov13} does not preclude 
achieving the bounds of Corollary \ref{short-cor:coreset-stream} in an adversarial
order (because our space is $\Ot(n^{1.5})$ rather than $\Ot(n)$),
the proof in~\cite{Kapralov13} (see
also~\cite{GoelKK12}) suggests that achieving such bounds is
ultimately connected to further understanding of \rs
graphs, a notoriously hard problem in additive combinatorics 
(see e.g. \cite{Gowers01, FoxHS15,AlonMS12}).
From a different perspective, 
most (but not all) streaming lower bounds are proven by bounding
the (per-player) communication complexity of the problem in the {blackboard communication model},
including the $\paren{\frac{e}{e-1}}$ lower bound of~\cite{Kapralov13}.
Our algorithm in Result~\ref{short-res:coresets} can be implemented with $\Ot(n)$ (per-player) communication in this model which goes strictly
below the lower bound of~\cite{Kapralov13}, thus establishing the first provable separation between
adversarial- and random-partitioned inputs in the blackboard model for approximating matchings.


\paragraph{\underline{Second implication: MPC.}} Maximum matching and minimum vertex cover are among the most studied graph optimization problems in the MPC and other MapReduce-style computation models
~\cite{AhnGM12Linear,LattanziMSV11,AhnG15,AssadiK17,CzumajLMMOS17,BehnezhadDETY17,HarveyLL18}. As an application of Result~\ref{short-res:coresets}, 
we obtain efficient MPC algorithms for matching and vertex cover in only two rounds of computation. 
 

\begin{corollary}\label{short-cor:coreset-mpc}
	There exist MPC algorithms that with high probability achieve a $(3/2+\eps)$-approximation to matching and a
        $(2+\eps)$-approximation to vertex cover in two MPC rounds and
         $\Ot(\sqrt{mn} + n)$ memory per machine\footnote{The approximation
          factor for vertex cover degrades to $4$ if one requires
          local computation on each machine to be polynomial time; see
          Remarks~\ref{rem:computational-time}
          and~\ref{rem:vc-polytime} in the full version.} for constant $\eps > 0$.
\end{corollary}

\noindent It follows from the results of \cite{AssadiKLY16} that sub-quadratic memory is not possible with one MPC round,
so two rounds is optimal. Furthermore, our implementation only requires one round if the
input is distributed randomly in the first place; see~\cite{MirrokniZ15} for details on when this assumption applies.


Our algorithms outperform the previous algorithms of~\cite{AssadiK17} for matching and vertex cover in terms of approximation ratio ($3/2$ vs.~$O(1)$ and $2$ vs.~$O(\log{n})$), while memory and round complexity are the same. Our matching algorithm outperforms the $2$-approximate maximum matching
algorithm of Lattanzi~\etal~\cite{LattanziMSV11} in terms of both the approximation ratio ($3/2$ vs. $2$) and round complexity ($2$ vs. $6$) within the same memory. Our result for the matching problem is particularly interesting 
as all other MPC algorithms~\cite{AhnGM12Linear,AhnG15,BehnezhadDETY17} that can achieve a better than two approximation (which is also a natural barrier for matching algorithms across different models) require a large (unspecified) constant
number of rounds. Achieving the optimal 2 rounds is significant in this context, since the round complexity of MPC algorithms determines the dominant cost of the computation (see, e.g.~\cite{LattanziMSV11,BeameKS13}), and hence 
minimizing the number of rounds is the primary goal in this model.


\paragraph{\underline{Third implication: distributed simultaneous communication.}} Maximum matching (and to a lesser degree vertex cover) has been studied previously in the 
simultaneous communication model owing to many applications of this model, including in achieving round-optimal distributed algorithms~\cite{AssadiK17}, proving lower bounds for dynamic graph streams~\cite{Konrad15,AiHLW16,AssadiKLY16,AssadiKL17}, 
and applications to mechanism design~\cite{DobzinskiNO14,AlonNRW15,Dobzinski16}. As an application of Result~\ref{short-res:coresets}, we obtain the following corollary. 
\begin{corollary}\label{short-cor:coreset-sim}
	There exist simultaneous communication protocols on randomly partitioned inputs that achieve $(3/2+\eps)$-approximation to matching and $(2+\eps)$-approximation to vertex cover with high probability
	(over the randomness of the input partitioning) with only $\Ot(n)$ communication per machine/player for constant $\eps > 0$. 
\end{corollary}

\noindent This result improves upon the $O(1)$ and $O(\log{n})$ approximation  of~\cite{AssadiK17} (on randomly partitioned inputs) for matching and vertex cover that were also designed by using randomized coresets. Our protocols 
achieve optimal communication complexity (up to $\polylog{(n)}$ factors)~\cite{AssadiK17}. 


\subsection{Second Result: MPC with Low Space Per Machine}\label{short-sec:result2}

Our second result concerns the MPC model with per-machine memory $O(n)$ or even $O(n/\polylog{(n)})$. This is achieved by 
extending our Result~\ref{short-res:coresets} from random edge-partitioned subgraphs (as in randomized coresets) to random vertex-partitioned subgraphs (which we explain further below).

\smallskip

\begin{result}\label{short-res:mpc}
	There exists an MPC algorithm that for any constant $\eps > 0$, with high probability, gives a $(1+\eps)$-approximation to maximum matching and $O(1)$-approximation to 
	minimum vertex cover in $O(\log\log{n})$ MPC rounds using only $O(n /\polylog{(n)})$ memory per 
	machine. 
\end{result}

Given an existing black-box reduction~\cite{LotkerPP15} (see also~\cite{CzumajLMMOS17}), our Result~\ref{short-res:mpc} immediately implies 
a $(2+\eps)$-approximation algorithm for maximum \emph{weighted} matching in 
the same $O(\log\log(n))$ rounds, though with the memory per machine increased to $O(n\log(n))$.

Prior to~\cite{CzumajLMMOS17}, all MPC
algorithms for matching and vertex cover~\cite{LattanziMSV11,AhnGM12Linear,AhnG15} 
required $\Omega\paren{\frac{\log{n}}{\log\log{n}}}$ rounds to achieve
$O(1)$ approximation when the memory per machine was restricted to
$\Ot(n)$ (which is arguably the most natural choice of parameter,
similar-in-spirit to the semi-streaming
restriction~\cite{FKMSZ05,M14}). 
In a very recent breakthrough, Czumaj~\etal~\cite{CzumajLMMOS17} presented an (almost) $2$-approximation algorithm for maximum matching that requires $O(n)$ (even $n/(\log{n})^{O(\log\log{n})}$) memory per machine
and only $O\paren{(\log\log{n})^2}$ MPC rounds. 
Result~\ref{short-res:mpc} improves upon this result on several fronts: $(i)$ we improve the round complexity of the matching algorithm
to $O(\log\log{n})$, resolving a conjecture of~\cite{CzumajLMMOS17} in the affirmative, $(ii)$ we obtain an $O(1)$ approximation to vertex cover, answering another open question of~\cite{CzumajLMMOS17}, and
$(iii)$ we achieve all these using a considerably simpler algorithm and analysis than~\cite{CzumajLMMOS17}.  

\paragraph{Comparison to results published after the appearance of our paper.}
After an earlier version of our paper was shared on arXiv \cite{AssadiBBMSarxiv2017}, Ghaffari et al.~\cite{GhaffariGMR18} presented a result very similar to 
our Result~\ref{short-res:mpc}: their bounds are exactly the same for matching, while for vertex cover they achieve a better
approximation in  the same asymptotic number of rounds: $(2+\eps)$-approximation vs. our $O(1)$ approximation. Techniques-wise, our approaches are entirely different: 
the algorithms in ~\cite{GhaffariGMR18} are based on an earlier round-compression technique of~\cite{CzumajLMMOS17},
and require an intricate local algorithm
and analysis to ensure consistency between machines;
see Section \ref{short-sec:techniques} below for more details.

Note that only our Result~\ref{short-res:mpc} is shared with the later paper of Ghaffari et al. \cite{GhaffariGMR18}: Result~\ref{short-res:coresets} appears only in our paper, and is entirely specific to the particular techniques that we use. 




\subsection{Our Techniques}\label{short-sec:techniques}

Both of our results are based on a novel
application of \emph{edge degree constrained subgraphs (EDCS)} that
were previously introduced by Bernstein and Stein~\cite{BernsteinS15}
for maintaining large matchings in dynamic graphs. 
Previous work
on EDCS~\cite{BernsteinS15,BernsteinS16} focused on how large a matching
an EDCS contains and how it can be maintained efficiently in a dynamic
graph. For the two results of this paper, we instead focus on the structural properties of the EDCS,
and prove several new facts in this regard.

For result~\ref{short-res:coresets}, we identify the EDCS as a sparse
certificate for large matchings and small vertex covers
which are quite robust to sampling and composition: an ideal
combination for a randomized coreset.
%
For Result~\ref{short-res:mpc}, we use the following recursive procedure, which
crucially relies upon on the robustness properties of the EDCS proved in 
Result~\ref{short-res:coresets}: we repeatedly compute an EDCS of the
underlying graph in a distributed fashion, redistribute it again 
amongst multiple machines, and recursively solve the problem on
this EDCS to compute an $O(1)$-approximation to matching and vertex
cover. We therefore limit the memory on each machine to only
$O(n)$ (even $O(n/\polylog{(n)})$) at the cost of increasing the number of rounds from $O(1)$ to
$O(\log\log{n})$.  Additional ideas are needed to ensure that the
approximation ratio of the algorithm does not increase beyond a fixed
constant as a result of repeatedly computing an EDCS of the current
graph in $O(\log\log{n})$ iterations.

%We obtain our coresets in Result~\ref{short-res:coresets} using a novel
%application of \emph{edge degree constrained subgraphs (EDCS)} that
%were previously introduced by Bernstein and Stein~\cite{BernsteinS15}
%for maintaining large matchings in dynamic graphs. While previous work
%on EDCS~\cite{BernsteinS15,BernsteinS16} focused on how large a matching
%an EDCS contains and how it can be maintained efficiently in a dynamic
%graph, in this paper we study several new structural
%properties of the EDCS itself. Our results identify these subgraphs as
%sparse certificates for large matchings and small vertex covers
%which are quite robust to sampling and composition, an ideal
%combination for a randomized  coreset.

\paragraph{Comparison of techniques.} 
Result~\ref{short-res:coresets} uses the definition of EDCS from \cite{BernsteinS15,BernsteinS16} but uses it in an entirely different setting, and hence we prove and use novel properties of EDCS in this work.

Result~\ref{short-res:mpc} relies on the high-level technique of
vertex sampling from Czumaj~\etal~\cite{CzumajLMMOS17}: instead
of partitioning the edges of the graph, each machine receives a
random sample of the vertices, and works on the resulting
induced subgraph.  Other than this starting point, our approach
proceeds along entirely different lines from~\cite{CzumajLMMOS17}, in
terms of both the local algorithm computed on each subgraph and in the
analysis.  The main approach in~\cite{CzumajLMMOS17} is \emph{round
  compression}, which corresponds to compressing multiple rounds of a
particular distributed algorithm into smaller number of MPC rounds by
maintaining a consistent state across the local algorithms computed on
each subgraph (using a highly non-trivial local algorithm and
analysis). Our results, on the other hand, do \emph{not} correspond to
a round compression approach at all and we do not require any
consistency in the local algorithm on each machine. Instead, we rely
on structural properties of the EDCS that we prove in this
paper, \emph{independent of the algorithms that compute these
  subgraphs}. This allows us to bypass many of the technical
difficulties arising in maintaining a consistent state across
different machines which in turn results in improved bounds and a
considerably simpler algorithm and analysis.

%After an earlier version of our paper was shared on arXiv \cite{AssadiBBMSarxiv2017}, Ghaffari et al. posted on arXiv a paper \cite{GhaffariGMR18} that (in addition to a second unrelated result) contains a result very similar
%to our Result~\ref{short-res:mpc}: their bounds are exactly the same for matching, while for vertex cover they achieve a better
%approximation in the same number of rounds: $(2+\eps)$-approximation vs. our $O(1)$. Techniques-wise, our approaches are entirely different: while the algorithms 
%in~\cite{GhaffariGMR18} are simpler than those of~\cite{CzumajLMMOS17}, they still
%rely on same round-compression framework, and thus require an intricate local algorithm and analysis
%to ensure a consistent state across machines.

\paragraph{Organization.} We present our notation and definitions of EDCS and the MPC model in Section~\ref{short-sec:prelim}. 
We then prove our structural results on
EDCS in Section~\ref{short-sec:edcs}. Section~\ref{short-sec:coresets-matching-vc} briefly describes how to prove Result~\ref{short-res:coresets} using these results. 
Finally, Section~\ref{short-sec:mpc-algs} contains the proof sketch of Result~\ref{short-res:mpc}. A full version of the paper containing omitted proofs and details appears at the end of the paper. 
In particular, we entirely postpone our new analysis of the randomized coreset of~\cite{AssadiK17} as well as a lower bound on its performance to Section~\ref{sec:maxmatching} of the full version but refer the reader to this result as 
a warm-up to our main results. Further related work are discussed in Section~\ref{sec:related} of the full version. 


%%\subsection{Related Work}\label{short-sec:related}
%%Maximum matching and minimum vertex cover are among the most studied problems in the context of massive graphs including in MPC model and MapReduce-style
%%computation~\cite{AhnGM12Linear,LattanziMSV11,AhnG15,AssadiK17,CzumajLMMOS17,BehnezhadDETY17}, streaming 
%%algorithms~{\cite{McGregor05,FKMSZ05,EKS09,EpsteinLMS11,AhnGM12Linear,GoelKK12,KonradMM12,AGM12,AG13,GO13,Kapralov13,KapralovKS14,CS14,ChitnisCHM15,M14,AhnG15,%
%%EsfandiariHLMO15,Konrad15,AssadiKLY16,ChitnisCEHMMV16,McGregorV16,EsfandiariHM16,AssadiKL17,PazS17}, simultaneous communication model and similar distributed 
%%models~\cite{GO13,DobzinskiNO14,HuangRVZ15,AlonNRW15,AssadiKLY16,AssadiKL17,AssadiK17}, dynamic graphs~\cite{NeimanS13,Solomon16,BaswanaGS15,OnakR10,BernsteinS15,BernsteinS16}, and 
%%sub-linear time algorithms~\cite{ParnasR07,HassidimKNO09,NguyenO08,OnakRRR12,YoshidaYI12}. 
%%Beside the results mentioned already, most relevant to our work are 
%%the $\polylog{(n)}$-space $\polylog{(n)}$-approximation algorithm of~\cite{KapralovKS14} for estimating the \emph{size} of a maximum matching in random stream, and the $(3/2)$-approximation
%%communication protocol of~\cite{GoelKK12} when the input is (adversarially) partitioned between two parties and the communication is from one party to the other one (as opposed to simultaneous which we studied). 
%%However, the techniques in these results and ours are completely disjoint. %We also remark that random partitioning of the input in communication models have been considered previously, for example in~\cite{ChakrabartiCM08}. 
%%
%%Coresets, composable coresets, and randomized composable coresets are respectively introduced in~\cite{AgarwalHV04},~\cite{IndykMMM14}, and~\cite{MirrokniZ15}. Composable coresets 
%%have been studied previously in nearest neighbor search~\cite{AbbarAIMV13}, diversity maximization~\cite{IndykMMM14,ZadehGMZ17}, clustering~\cite{BalcanEL13,BateniBLM14}, and
%%submodular maximization~\cite{IndykMMM14,MirrokniZ15,BadanidiyuruMKK14,BarbosaENW15,BarbosaENW16}. Moreover, while not particularly termed a composable coreset, the ``merge and reduce'' technique
%%in graph streaming literature (see~\cite{M14}, Section~2.2) is identical to composable coresets. 

%Finally similar ideas as randomized coreset for optimization problems has also been used in random arrival streams~\cite{KonradMM12,KapralovKS14}. 


%%
%%MapReduce computation, and different distributed computation models. 
%%Most relevant to our work are the linear sketches of~\cite{ChitnisCEHMMV16} for computing an \emph{exact} minimum vertex cover or maximum matching in $O(\opt^2)$ space ($\opt$ is the size of the solution), and linear
%%sketches of~\cite{AssadiKLY16,ChitnisCEHMMV16} for $\alpha$-approximating maximum matching in $\Ot(n^2/\alpha^3)$ space. These results are proven to be tight by~\cite{ChitnisCHM15}, and~\cite{AssadiKLY16}, respectively.
%%Finally,~\cite{AssadiKLY16} also studied the simultaneous communication complexity of bipartite matching in the vertex-partition model and proved that obtaining better than an $O(\sqrt{k})$-approximation in this model 
%% requires strictly more than $\Ot(n)$ communication from each player (see~\cite{AssadiKLY16} for more details on this model). 

%%Coresets, composable coresets, and randomized composable coresets are respectively introduced in~\cite{AgarwalHV04},~\cite{IndykMMM14}, and~\cite{MirrokniZ15}. Composable coresets 
%%have been used previously in the context of nearest neighbor search~\cite{AbbarAIMV13}, diversity maximization~\cite{IndykMMM14}, clustering~\cite{BalcanEL13,BateniBLM14}, and
%%submodular maximization~\cite{IndykMMM14,MirrokniZ15,BadanidiyuruMKK14}. Moreover, while not particularly termed a composable coreset, the ``merge and reduce'' technique
%%in graph streaming literature (see~\cite{M14}, Section~2.2) is identical to composable coresets. Finally similar ideas as randomized coreset for optimization problems has also been used in random arrival streams~\cite{KonradMM12,KapralovKS14}. 
%%
%%




 



==> mpc-algorithms-short.tex <==

\section{MPC Algorithms for Matching and Vertex Cover}\label{short-sec:mpc-algs}
%%\todo[inline]{For the shortened version, I would simply remove this entire paragraph, as well as the repetition of the Theorem.}
%%As was shown in Section~\ref{sec:coreset}, our randomized coresets for matching and vertex cover in Section~\ref{sec:coresets-matching-vc} immediately imply MPC algorithms for these problems in only two MPC rounds. 
%%However, while quite round-efficient, the memory requirement of these algorithms can be as large as $\Theta(n\sqrt{n})$ in case of dense input graphs. In this section, we show that a careful adaptation of our coresets construction together 
%%with the structural results proven for EDCS in Section~\ref{sec:edcs} can be used to obtain MPC algorithms with memory requirement of $\Ot(n)$ while increasing the number of required rounds to only $O(\log\log{n})$. Formally, we show that, 
%%
%%\begin{theorem}\label{thm:mpc-matching-vc}
%%	There exists an MPC algorithm that given a graph $G(V,E)$ with high probability computes an $O(1)$ approximation to both maximum matching and minimum vertex cover of $G$ in $O(\log\log{n})$ MPC rounds using only $\Ot(n)$ memory per 
%%	machine. 
%%\end{theorem}

%We sketch the proof of Result~\ref{short-res:mpc} in this section. 

In this section, we show that a careful adaptation of our coresets construction together 
with the structural results proven for EDCS in Section~\ref{short-sec:edcs} can be used to obtain MPC algorithms with much smaller memory while increasing the number of required rounds to only $O(\log\log{n})$. 

\begin{theorem}\label{short-thm:mpc-matching-vc}
	There exists an MPC algorithm that given a graph $G(V,E)$ with high probability computes an $O(1)$ approximation to both maximum matching and minimum vertex cover of $G$ in $O(\log\log{n} + \log{\paren{\frac{n}{s}})}$ MPC rounds
	 on machines of memory $s = n^{\Omega(1)}$.
\end{theorem}

By setting $s = O(n/\polylog{(n)})$ in Theorem~\ref{short-thm:mpc-matching-vc}, we achieve an $O(1)$-approximation algorithm to both matching and vertex cover in $O(\log\log{n})$ MPC rounds on machines of memory $O(n/\polylog{(n)})$, formalizing Result~\ref{res:mpc} (reducing the approximation ratio to $(1+\eps)$ for matching can be done by adapting the reduction of~\cite{McGregor05} from streaming to MPC model; see Section~\ref{sec:mpc-matching-1} in full version for details). 

In the following, for the sake of clarity, we focus on sketching the proof of Theorem~\ref{short-thm:mpc-matching-vc} for the natural case when memory per machine is $s = \Ot(n)$. (See Section~\ref{sec:mpc-smaller-memory} of full version
for the additional (standard) ideas needed to reduce the memory to any $s = n^{\Omega(1)}$ at a cost of increasing the number of the rounds by an additive $O(\log{\paren{\frac{n}{s}})}$ factor);
The overall idea of the algorithm in this result is as follows. 
Instead of the edge sampled subgraphs used by our randomized coresets, we start by picking $k = O(n)$ \emph{vertex} sampled subgraphs of $G$ with sampling probability roughly $1/\sqrt{n}$ 
and send each to a separate machine. 
Each machine then locally computes an EDCS of its input (with parameters $\beta = \polylog{(n)}$ and $\beta^- \approx \beta$) with no coordination across the machines. Unlike the MPC algorithm obtained 
by our randomized coreset approach (Corollary~\ref{short-cor:coreset-mpc}), where the memory per machine was as large as $\Theta(n\sqrt{n})$, here we cannot collect all these smaller EDCSes on a single machine of memory $\Ot(n)$. 
Instead, we repartition them across the machines again (and discard remaining edges) and repeat the previous process on this new graph. The main 
observation is that after each step, the maximum degree of the remaining graph (i.e., the union of all EDCSes) would drop quadratically (e.g., from $\Omega(n)$ to $\Ot(\sqrt{n})$ in the first step). As such, in each subsequent step, 
we can pick a smaller number of vertex sampled subgraphs, each with a higher sampling probability than previous step, and still each graph fits into the memory of a single machine. Repeating this process for $O(\log\log{n})$ steps reduces the maximum degree of the remaining graph
to $\polylog{(n)}$. At this point, we can store the final EDCS on a single machine and solve the problem locally. 

Unfortunately this approach on its own would only yield a $(3/2)^{O(\log\log{n})} = \polylog{(n)}$ approximation to matching, since by Lemma \ref{short-lem:edcs} each recursion onto an EDCS
of the graph could introduce a $3/2$-approximation.
A similar problem exists for vertex cover. In the proof of 
Lemma \ref{short-lem:edcs}, computing a vertex cover of $G$ from its EDCS $H$ involves two steps: we
add to the vertex cover all vertices with high degree in $H$ to cover the edges in $G \setminus H$,
and then we separately compute a vertex cover for the edges in $H$. Since $H$ cannot fit into a single machine, the second computation is done recursively: in each round, we find an EDCS of the current graph (which is partitioned amongst many machines), add to the vertex cover all high degree vertices in this EDCS, and then recurse onto the sparser EDCS. A straightforward analysis would only lead
to an $O(\log\log{n})$ approximation. 

We improve the approximation factor for both vertex cover
and matching by showing that they can serve as witnesses to each other. Whenever we
add high-degree vertices to the vertex cover, we will also find a large matching incident to these
vertices; this can be done in $O(1)$ parallel rounds. We then argue
that their sizes are always within a constant factor of each other, which is well known to imply that both are a constant approximation for the respective problem 
(see Proposition~\ref{prop:vc-matching-alpha}).

The rest of this section is organized as follows. We first describe the subroutines for computing an EDCS from vertex sampled subgraphs and for 
obtaining a large matching incident on high degree vertices. 
We then combine these subroutines to provide our main parallel algorithm. The MPC implementation details of our algorithm as well as extension of the maximum matching algorithm to 
$(2+\eps)$ and $(1+\eps)$-approximation is deferred to Section~\ref{sec:mpc-implementation} and Section~\ref{sec:mpc-wrap-up} of the full version.  

\paragraph{Main Subroutines.} In the following two subroutines, both the input graph and the output edges are distributed across multiple machines. The formal description of these subroutines and the proofs of their correctness are presented in Section~\ref{sec:mpc-edcs} and Section~\ref{sec:random-match} of the full version.
\begin{tbox}
$\pedcs(G,\Delta)$. A parallel algorithm for computing an EDCS of a given graph $G$ with maximum degree $\Delta$ on machines of memory $\Ot(n)$. With high probability, the computed EDCS has parameters 
	$\beta = O(\sqrt{\Delta}) \cdot \polylog{(n)}$ and $\beta^- \geq 0.99 \cdot \beta$ and is edge-partitioned across multiple machines. 
\end{tbox}
\begin{tbox}
	$\rmatch(G,S,\Delta)$. Let $G$ be a graph with maximum degree $\Delta$ and let $S$
	be a set of vertices with degree at least $\Delta/3$ in $G$. $\rmatch(G,S,\Delta)$
	is a parallel algorithm running on machines of memory $n^{\Omega(1)}$ that finds a matching $M$
	such that every edge in $M$ is incident to $S$, and  
	$\Ex\card{M} = \Theta(\card{S})$. (The existence of such a large matching in $G$ follows from basic facts in graph theory; see Proposition~\ref{prop:matching-high-degree}.) 
\end{tbox}

We briefly describe the main ideas behind each of these subroutines. $\pedcs(G,\Delta)$ works by creating $O(\Delta)$ vertex sampled subgraphs of $G$ with sampling probability roughly $1/\sqrt{\Delta}$, each on
a separate machine. It is easy to see that the total number of edges in each such subgraph is at most $\Ot(n)$ with high probability and hence this graph fits the memory of a single machine. Each machine then computes an EDCS of its input with parameters $\beta = \polylog{(n)}$ and $\beta^- \approx \beta$. Similar to 
Section~\ref{short-sec:coresets-matching-vc}, we can prove that the union of these edges is an EDCS of the original graph with the aforementioned parameters (this time using Lemma~\ref{short-lem:edcs-vertex-sampled} for vertex sampled subgraphs). 

$\rmatch(G,S,\Delta)$ is based on a simple randomized procedure. The machines collectively sample each edge incident to $S$ in $G$ with probability $1/\Delta$ independently, and then add all edges with \emph{unique endpoints} in this process
to the final matching $M$ (these edges can be found in parallel using a parallel sort subroutine).
Since degree of vertices in $G$ is at most $\Delta$, while degree of vertices in $S$ is at least $\Delta/3$, one can show
that the expected size of the matching returned is $\Omega(\card{S})$. 
\paragraph{Parallel Algorithm for Matching and Vertex Cover.} 
We now present our main algorithm. 

\textbox{\textnormal{$\palg(G,\Delta)$. A parallel algorithm for computing a vertex cover $\va$ and a matching $\ma$ of a given graph $G$ with maximum degree at most $\Delta$. }}{

	\begin{enumerate}
		\item If $\Delta \leq \paren{400 \cdot \log^{12}{n}}$ send $G$ to a single machine;  compute a maximal matching $\ma$ in $G$ and let $\va$ be the set of vertices matched by $\ma$. 
		Return $\va$ and $\ma$. Otherwise, continue the following algorithm. 
	%	\item If $\Delta > \paren{400 \cdot \log^{12}{n}}$, we run the following algorithm. 
		\item Compute an EDCS $C := \pedcs(G,\Delta)$ in parallel. Let $\beta_C = O(\sqrt{\Delta}) \cdot \polylog{(n)}$, and $\beta^-_C = 0.99 \cdot \beta_C$ be the parameters of this EDCS. % (as specified in Claim~\ref{clm:palg-pedcs} below). 
		  %compute an $\EDCS{G,\beta_C,\beta^-_C}$ (for parameters $\beta_C,\beta^-_C$ defined in Lemma~\ref{lem:edcs-vertex-partition}) denoted by $$.
		\item Define $\vh := \set{v \in V \mid \deg{C}{v} \geq \beta^-_C/2}$ be the set of ``high'' degree vertices in $C$. 
		\item Compute a matching $\mh := \rmatch(C,\vh,\beta_C)$. 
		\item Define $\vm := V \setminus \Paren{\vh \cup V(\mh)}$ as the set of vertices that are neither high degree in $C$ nor matched by $\mh$. Let $\cm$ be the induced subgraph of $C$ on vertices $\vm$.
		\item Recursively compute $(\vr,\mr) := \palg(\cm, \beta_C)$. 
		\item Return $\va := \vh \cup V(\mh) \cup \vr$ and $\ma := \mh \cup \mr$. 
	\end{enumerate}	
}

The total number of recursive calls made by $\palg(G,\Delta)$ is $O(\log\log{\Delta})$ as the maximum degree of the underlying graph drops from $\Delta$ to $\Ot(\sqrt{\Delta})$ after 
each call (see Claim~\ref{clm:palg-steps} in the full version). The detailed proof of the following lemma appears in Section~\ref{sec:mpc-main} of the full version. 

%We are ready to prove the correctness of $\palg$. 
\begin{lemma}\label{short-lem:palg-correct}
	For any graph $G(V,E)$, $\palg(G,n)$, with constant probability, outputs a matching $\ma$ which is an $O(1)$-approximation to the maximum matching of $G$ and a vertex cover $\va$ which is an $O(1)$-approximation to the minimum vertex cover of $G$. 
\end{lemma}
\begin{proof}[Proof Sketch.]
	In the following, we assume that all the calls made to \pedcs and \rmatch in $\palg$ return a correct answer which happens
	with high probability by a union bound. 
	We first argue that $\va$ and $\ma$ are respectively a feasible vertex cover and a feasible matching of $G$ with high probability. The case for $\ma$ is straightforward; the set of vertices matched by $\mh$ is disjoint from the vertices in 
	$\mr$ as all vertices matched by $\mh$ are removed in $\cm$, and hence (by induction) $\ma = \mh \cup \mr$ is a valid matching in $G$. Now consider the set of vertices $\va$. Since 
	$C$ is an $\EDCS{G,\beta_C,\beta^-_C}$, by \proptwo of EDCS $C$, any edge $e \in G \setminus C$ has at least one neighbor in $\vh$ and is thus covered by $\vh$. 
	Additionally, as we pick $V(\mh)$ in the vertex cover, any edge incident on these vertices is also covered. Thus $\vh \cup V(\mh)$ covers all edges in $G \setminus C^-$, and (by induction) $\vr$
	covers all the edges in $C^-$

	We now show that the sizes of $\ma$ and $\va$ are within a constant factor of each other in expectation, which is well known to imply that both are an $O(1)$-approximation to their respective problem (see Proposition~\ref{prop:vc-matching-alpha}). 
	By correctness of $\rmatch$, $\vh$ and $\mh$ are within a constant factor of each other in expectation. Moreover, clearly $\card{V(\mh)} \leq 2\card{\vh}$, so the vertex cover $\vh \cup V(\mh)$ and the matching $\mh$ chosen at each step are within a 
	constant factor of each other. By induction, the final outputs $\va$ and $\ma$ are also within a constant factor of each other in expectation. This, together with a simple application of Markov bound ensures
	that with probability $\Omega(1)$, $\va$ and $\ma$ are an $O(1)$-approximation to their respective problem. 
\end{proof}

We note that in Lemma~\ref{short-lem:palg-correct}, we only achieved a constant factor probability of success for $\palg$. We can however run this algorithm in parallel $O(\log{n})$ times and pick the best solution to achieve a high probability of success while still 
having $\Ot(n)$ memory per machine and $O(\log\log{n})$ rounds. In Sections~\ref{sec:mpc-palg-machines} and~\ref{sec:mpc-smaller-memory} of full version, 
we further discuss optimizing the number of machines and the per-machine memory of this algorithm, respectively. 







==> prelim-short.tex <==


\smallnegsp

\section{Preliminaries}\label{short-sec:prelim}

\paragraph{Notation.} For a graph $G(V,E)$, we use $\MM(G)$ to denote the maximum matching size in $G$ and $\VC(G)$ to denote the minimum vertex cover size. 
%%For any subset of vertices $V' \subseteq V$ and any subset of edges $E' \subseteq E$, we use $V'(E')$ to denote the set of vertices in $V'$ that are incident on edges of $E'$ and 
%%$E'(V')$ to denote the set of edges in $E'$ that are incident on vertices of $V'$. 
For any vertex $v \in V$, $\deg{G}{v}$ denotes the degree of $v$ in the graph $G$. 
%We use capital letters to denote random variables.  A summary of concentration bounds that we use in this paper appears in Appendix~\ref{app:concentrations}. 


\paragraph{Sampled Subgraphs.} We use two different ways of sampling a graph $G(V,E)$. For $p \in (0,1)$, 
\begin{itemize}
	\item A graph $\GEp(V,E_p)$ is an \emph{edge sampled subgraph} of $G$ iff the vertex set of $\GEp$ and $G$ are the same and every edge in $E$ is picked independently and with probability $p$ in $E_p$. 
	\item A graph $\GVp(V_p,E_p)$ is a \emph{vertex sampled (induced) subgraph} of $G$ iff every vertex in $V$ is sampled in $V_p$ independently and with probability $p$ and $\GVp$ is the induced subgraph of $G$ on $V_p$
\end{itemize}


\paragraph{The Massively Parallel Computation (MPC) Model.}%\label{sec:mpc} 
We adopt the most stringent model of modern parallel computation among~\cite{KarloffSV10,GoodrichSZ11,AndoniNOY14,BeameKS13}, the so-called \emph{Massively Parallel Computation (MPC)} model of~\cite{BeameKS13}. 
Let $G(V,E)$ with $n:= \card{V}$ and $m := \card{E}$ be the input graph. 
In this model, there are $p$ machines, each with a memory of size $s$. One typically requires that both $p,s = m^{1-\Omega(1)}$ i.e., polynomially smaller than the input size~\cite{KarloffSV10,AndoniNOY14}. 
% such that $p \cdot s = \Ot(m)$. 
Computation proceeds in synchronous rounds: in each round, each machine performs some local computation
and at the end of the round machines exchange messages. All messages sent and received by each machine in each round have to fit into the local memory of the machine. This in particular means that
the length of the messages on each machine is bounded by $s$ in each round. At the end, the machines collectively output the solution. 

%%\subsection{Basic Graph Theory Facts} \label{sec:graph-facts}
%%
%%\begin{fact}\label{fact:vc-matching}
%%	For any graph $G(V,E)$, $\MM(G) \leq \VC(G) \leq 2 \cdot \MM(G)$. 
%%\end{fact}
%%
%%The  following propositions are well-known and are proven in Appendix~\ref{app:graph-facts} for completeness. 
%%\begin{proposition}\label{prop:vc-matching-alpha}
%%	Suppose $M$ and $V'$ are respectively, a matching and a vertex cover of a graph $G$ such that $\alpha \cdot \card{M} \geq \card{V'}$; then, both $M$ and $V'$ are $\alpha$-approximation 
%%	to their respective problems. 
%%\end{proposition}
%%%%\begin{proof}
%%%%	$\VC(G) \Geq{Fact~\ref{fact:vc-matching}} \MM(G) \geq \card{M} \geq \frac{1}{\alpha} \cdot \card{V'} \geq \frac{1}{\alpha} \cdot \VC(G) \Geq{Fact~\ref{fact:vc-matching}} \frac{1}{\alpha} \cdot \MM(G)$. 
%%%%\end{proof}
%%
%%\begin{proposition}\label{prop:matching-high-degree}
%%	Suppose $G(V,E)$ is a graph with maximum degree $\Delta$ and $\vh$ is the set of all vertices with degree at least $\gamma \cdot \Delta$ in $G$ for $\gamma \in (0,1)$. Then,  $\MM(G) \geq \frac{\gamma \cdot \Delta}{\Delta+1} \cdot \card{\vh}$. 
%%\end{proposition}
%%%%\begin{proof}
%%%%	By Vizing's theorem~\cite{Vizing64}, $G$ can be edge colored by at most $D + 1$ colors. As each color class forms a matching, this means that there exists a matching $M$ in $G$ with $\card{M} \geq \frac{\card{E}}{D + 1}$. Moreover, 
%%%%	we have $\card{E} \geq \card{\vh} \cdot \gamma \cdot D$, finalizing the proof. 
%%%%\end{proof}

\paragraph{Edge Degree Constrained Subgraph (EDCS).} We introduce edge degree constrained subgraphs (EDCS) in this section and present several of their properties which are proven in previous work. \emph{We emphasize that all other properties of EDCS proven in the subsequent sections 
are new to this paper.} An EDCS is defined formally as follows. 

\begin{definition}[\!\!\cite{BernsteinS15}]\label{short-def:edcs}
	For any graph $G(V,E)$ and integers $\beta \geq \beta^- \geq 0$, an \emph{edge degree constraint subgraph (EDCS)} $(G,\beta,\beta^-)$ is a subgraph $H:=(V,E_H)$ of $G$ with the following two properties: 
	\begin{enumerate}[(P1)]
		\item For any edge $(u,v) \in E_H$: $\deg{H}{u} + \deg{H}{v} \leq \beta$. 
		\item For any edge $(u,v) \in E \setminus E_H$: $\deg{H}{u} + \deg{H}{v} \geq \beta^-$.  
	\end{enumerate}
%	We sometimes abuse the notation and use $H$ and $E_H$ interchangeably. 
\end{definition}


In the remainder of the paper, we use the terms ``\propone'' and ``\proptwo'' of EDCS to refer to the first and second items in Definition~\ref{short-def:edcs} above. 

Previous work in~\cite{BernsteinS15,BernsteinS16} has shown that for any choice of $\beta^- < \beta$, an $\EDCS{G,\beta,\beta^-}$ always exists (see Lemma~\ref{lem:edcs-exists} in the full version). 
Moreover, it was shown in~\cite{BernsteinS15} (bipartite graphs) and~\cite{BernsteinS16} (general graphs)
that an EDCS accurately preserves the maximum matching in $G$. It is easy to show a qualitatively similar result
for vertex cover. We summarize these results in the lemma below (see Lemmas~\ref{lem:edcs-matching} and \ref{lem:edcs-vc} in the full version for a more thorough discussion).

\begin{lemma}[\!\!\cite{BernsteinS15,BernsteinS16}]\label{short-lem:edcs}
Consider any parameters $\eps > 0$, $\beta = \Omega(\eps^{-3})$ and 
$\beta^- = (1-\Theta(\eps)) \cdot \beta$. If $H$ is an $\EDCS{G,\beta,\beta^-}$ of $G$
then: 
{\bf (1)} $\MM(G) \leq (3/2 + \eps) \cdot \MM(H)$ and 
{\bf (2)} given only the graph $H$, one can recover a $(2+\eps)$-approximation to $\VC(G)$ 
without further access to the original graph $G$.
\end{lemma}

\begin{proof}[Proof Sketch.]
The proof that $\MM(G) \leq (3/2 + \eps) \cdot \MM(H)$ is presented in \cite{BernsteinS15,BernsteinS16} 
and requires a fairly complicated argument. 
%and is quite complicated. 
The proof for vertex cover however is simpler.
The basic idea is that we start with $\VC(H)$ to cover the edges of $H$,
and then by \proptwo of EDCS $H$ we can cover edges in $G \setminus H$ by 
adding to the vertex cover all vertices $v$ with $d_H(v) \geq \beta^-/2$.
\end{proof}







